Federated Whole Prostate Segmentation in MRI with Personalized Neural Architectures

Building robust deep learning-based models requires diverse training data, ideally from several sources. However, these datasets cannot be combined easily because of patient privacy concerns or regulatory hurdles, especially if medical data is involved. Federated learning (FL) is a way to train machine learning models without the need for centralized datasets. Each FL client trains on their local data while only sharing model parameters with a global server that aggregates the parameters from all clients. At the same time, each client's data can exhibit differences and inconsistencies due to the local variation in the patient population, imaging equipment, and acquisition protocols. Hence, the federated learned models should be able to adapt to the local particularities of a client's data. In this work, we combine FL with an AutoML technique based on local neural architecture search by training a "supernet". Furthermore, we propose an adaptation scheme to allow for personalized model architectures at each FL client's site. The proposed method is evaluated on four different datasets from 3D prostate MRI and shown to improve the local models' performance after adaptation through selecting an optimal path through the AutoML supernet.

==> old_miccai2020/01_Introduction.tex <==
% TODO:
%Statistical testing. 
%What are the different networks

\section{Introduction}
\label{sec:intro}
The advancements of the last few years in medical image segmentation were dominated by deep learning (DL) approaches. DL mostly replaced the need for handcrafting of image features. However, one could argue that it has replaced it with the need to hand-engineer different network architectures. In particular, the medical image computing field has been dominated by popular hand-engineered network architectures such as 2D and 3D U-Net \cite{ronneberger2015u,cciccek20163d}, V-Net \cite{milletari2016v}, High-Res-Net \cite{li2017compactness}, DeepMedic \cite{kamnitsas2016deepmedic}, and many others. One potential solution to reduce the amount of engineering required by DL domain experts is through the application of automated machine learning (``AutoML'') techniques.
%
%\paragrah{Federated Learning Background:}
At the same time, DL requires massive amounts of data to train robust models. Often hospitals and other medical institutes need to collaborate and host centralized databases for the development of clinical-grade DL models. This can become very challenging due to data-privacy and various ethical concerns associated with data sharing in healthcare. One approach to combat the data sharing and privacy issues is through federated learning (FL), where only model gradients are shared between participating institutes but no raw data.
%
Furthermore, it is well known that models trained on large centralized datasets might not always generalize well to the distribution of the data at a particular imaging site due to various inconsistencies (scanner, imaging protocols, patient population, etc.) between the different sites. In this case, domain adaptation (DA) methods need to be developed which can adapt the model to the local particularities of the data. 
%
In this work, we aim to address these three problems simultaneously by combining an FL algorithm with AutoML approaches for local model adaptation. In particular, we implement a ``supernet'' training strategy that can be trained in a federated setting.
%
We feel that AutoML and FL technologies are a perfect fit for each other because of their complementary nature. By combining the two, we are also able to address the DA problem. %
For one, FL can circumvent the problem of hosting and accessing large centralized datasets by distributing the learning effort to several clients with their own local data. FL will only communicate the model gradients after a local round of training to a centralized server which aggregates the results and starts the next round of FL.
%
At the same time, AutoML allows us to avoid hand-engineering of dataset-specific network architectures and a particular sub-network of the trained supernet can be used as a way of local domain adaptation to handle inconsistencies between the different contributing data sites. 

\subsection{Related Works}
\label{related_works}
\paragraph{\textbf{Automl:}}
Recently, for various applications, such as image recognition, semantic segmentation, object detection, natural image generation, etc., the AutoML approaches for DL have been explored. However, often very particular network architectures need to be hand-designed for each task. Neural architecture search (NAS)~\cite{elsken2018neural} is one of the most common approaches to circumvent the hand-design of architectures in AutoML for DL applications. The goal of NAS is to automatically design neural network architectures without any human heuristics or assumptions. In addition to the model weights, after searching, the model architecture itself optimized for the task at hand, while often still being generalizable to other datasets \cite{yu2019c2fnas}. 
%
A common concept in NAS and AutoML literature is the ``supernet'' \cite{liu2018darts,guo2019single,cai2018proxylessnas,wu2019fbnet,shaw2019squeezenas}. The main idea behind supernet is that we can create a large neural network including several candidate modules at each level of the networks. This supernet can be trained jointly or specific sub-networks can be chosen by selecting a path through the module candidates. At deployment, the final architecture is selected from the supernet by assigning path weights to select particular module candidates.
%
Additional budgeting constraints, such as latency or number of model parameters, can be added to find optimal architectures for a given application. Recent works can achieve state-of-the-art results on computer vision tasks while being computationally efficient \cite{tan2019efficientnet}.

\paragraph{\textbf{Federated Learning:}}
FL enables collaborative and decentralized DL training without sharing raw patient data \cite{mcmahan2016communication}. Each client in FL trains locally on their own data and then submits their model parameters to a server that accumulates and aggregates the model updates from each client. Once a certain number of clients have submitted their updates, the aggregated model parameters are redistributed to the clients and a new round of local training starts. While out of the scope of this work, FL can also be combined with additional privacy-preserving measures to avoid potential reconstruction of training data through model inversion if the model parameters would be leaked to an adversary \cite{li2019privacy}. Recent works have shown the applicability of FL to medical imaging tasks \cite{sheller2018multi,li2019privacy}. 

\paragraph{\textbf{Domain adaptation:}}
Researchers have suggested many approaches to domain adaptation to tackle data inconsistencies generated by unknown data or different domains. In its simplest form, fine-tuning, also known as transfer learning \cite{shin2016deep}, can help to adapt a pre-trained model to a particular target domain. 
More recent approaches for DA typically involve some form of adversarial learning to introduce a specific loss that can minimize the feature-level differences between different domains \cite{kamnitsas2017unsupervised} or through gradient back-propagation using adversarial training~\cite{ganin2015unsupervised,ganin2016domain}.
An alternative approach is coming from the ``image translation'' field where generative adversarial networks (GAN) are utilized to translate the image of one domain to mimic another domain. An important part of these approaches is the application of some form of cycle-consistency which is essential to train on un-paired data \cite{isola2017image,zhu2017unpaired,zhang2018task}
The common concept of adversarial training suggests that the gradients from external constraints will help balance various domains and change the model's feature representations.

Our proposed approach here is similar in that we will ultimately adapt the model's internal feature representations through the selection of an adapted sub-network of the trained supernet, but without needing to use computationally expensive adversarial learning schemes.

\subsection{Contributions}
Our contributions can be summarized as follows:
\begin{enumerate}
    \item We show that we can successfully train models through federated learning with comparable performance to models trained on centrally hosted data.
    \item We extent federated learning by introducing an AutoML approach for supernet model training.
    \item We show that finding an optimal path through the supernet can act as a form of local domain adaptation and bring performance gains.
\end{enumerate}


==> old_miccai2020/02_Methods.tex <==
\section{Method}
\label{sec:method}
Here we describe the technical details of the FL and AutoML approach utilized in this work. 
The proposed method can be separated into two steps: 1) FL with AutoML supernet training and 2) local model adaptation by finding the best path through the supernet with respect to the local data. Both FL and AutoML procedures presented are designed for 3D medical image segmentation tasks.

\subsection{Client-Server-Based Federated Learning}
In its typical form, FL utilizes a client-server setup. Each client trains the same model architecture locally on their own data. Once a certain number of clients finished local training, the updated model weights (or their gradients) are sent to the server for aggregation. After aggregation, the new weights on the server are re-distributed to the clients and the next round of local model training is executed. After several FL rounds, the models at each client are converged. Each client can be allowed to select their locally best model by monitoring a certain performance metric on a local hold out validation set. In our experiments, we implement the \texttt{FederatedAveraging} algorithm proposed in \cite{mcmahan2016communication}. While there exist variations of this algorithm to address particular learning tasks, in its most general form, FL tries to minimize a global loss function $\mathcal{L}$ which can be a weighted combination of $K$ local losses $\{\mathcal{L}_k\}_{k=1}^{K}$ that each is computed on a client $k$'s local data.
Hence, FL can be formulated as the task of finding the model parameters $\phi$ that minimize $L$ given some local data $X$.
%
\begin{align}
\min_{\phi}\mathcal{L}(X; \phi) \quad \text{with} \quad  \mathcal{L}(X; \phi)=\sum_{k=1}^{K}w_{k}\;\mathcal{L}_{k}(X_{k}; \phi),
\label{eq:formalism}
\end{align}
%
where $w_k>0$ denote the weight coefficients for each client $k$, respectively. Note, that the local data $X_{i}$ is never shared among the different clients. Only the model weights are accumulated and aggregated on the server as shown in Algorithm~\ref{alg:fl}.
\begin{algorithm}[htb]
\caption{Client-server federated learning with \texttt{FederatedAveraging}~\cite{mcmahan2016communication,li2019privacy}. $T$ is the number of federated learning rounds and $n_k$ is the number of \texttt{LocalTraining} iterations minimizing the local loss $\mathcal{L}_{k}(X_{k}; \phi^{(t-1)})$ for a client $k$.}
\label{alg:fl}
\small
%
  \begin{algorithmic}[1]
    %\Require{Number federated round $T$}
    %\Require{Number of local training iterations $n_k$}
    \Procedure{Federated Learning}{}
      \State{Initialize weights: $\phi^{(0)}$}
      \For{$t \gets 1\cdots T$}
        \For{$client\ k \gets 1\cdots K$}  \Comment{ \textit{Executed in parallel}}
        \State{Send $\phi^{(t-1)}$ to client $k$}
        \State{Receive $(\Delta \phi_k^{(t)}, n_k)$ from client's $\texttt{LocalTraining}(\phi^{(t-1)})$}
        %\Comment{\textit{Minimizing} $\mathcal{L}_{k}(X_{k}; \phi^{(t-1)})$}} 
        \EndFor
        \State{$\phi_k^{(t)}\gets \phi^{(t-1)} + \Delta \phi_k^{(t)}$}
        \State{$\phi^{(t)}\gets \frac{1}{\sum_k{n_k}}\sum_k{(n_k\cdot \phi_k^{(t)})}$}
      \EndFor
      \State \Return $\phi^{(t)}$
  \end{algorithmic}
\end{algorithm}

\subsection{AutoML with Supernet}
We designed a supernet $\mathcal{S}$ consisting of various DL module candidates $\mathcal{M}$ suitable for 3D medical imaging tasks shown in Table \ref{tab:candidates}. These modules are optimized at multiple resolution levels to capture different levels of low-level and more semantic image features useful for the segmentation task. In general, we follow the popular encoder-decoder structure which has been successfully applied to many medical imaging tasks \cite{ronneberger2015u,cciccek20163d,milletari2016v} as shown in Fig. \ref{fig:supernet} with skip connections that concatenate features of the encoder with their corresponding layer in the decoder path.
During training, we choose arbitrary paths $m$ from the module candidates $\mathcal{M}$ following a uniform sampling scheme (see Fig. \ref{fig:modules}) to define a sub-network $s$ sampled from the supernet $\mathcal{S}$.

In this work, we choose the Dice loss \cite{milletari2016v} as our loss function which is commonly used for segmentation tasks in medical imaging. Its major advantage is its ability to work well in segmentation tasks with an unbalance in the amount of foreground/background regions:
\begin{equation}
    \min_{s \in \mathcal{S}} \left( \mathcal{L}_{Dice} \right) =
    \left(  1 - \frac{2\sum_{i=1}^{N}p_ig_i}{\sum_{i=1}^{N} p_i^2 + \sum_{i=1}^{N} g_i^2}
    \label{eq:dice_loss}  \right)
    ,
\end{equation}
Here, $p_i$ is the predicted probability from the final \textit{sigmoid} activated output layer of our supernet network $f(X)$ and $g_i$ is the ground truth label map at a given voxel $i$.

Once the supernet is trained, we can find a locally optimal path for a sub-network $s_0$ through the supernet, effectively adapting the model to the target domain. During adaptation, the model parameters $\phi$ stay fixed and only the path weights are optimized for one epoch on the local validation set. This results in an optimal path $m_0 \in \mathcal{M}$ that defines our locally adapted sub-network $s_0 \in \mathcal{S}$.

\begin{figure}[htbp]
 \centering
    \subfloat[(a)]{
        \includegraphics[width=0.6\textwidth,valign=c]{figs/supernet.png} 
        \label{fig:supernet}
    }%
    %\qquad
    \subfloat[(b)]{
        \includegraphics[width=0.3\textwidth,valign=c]{figs/modules.png}
        \label{fig:modules}
    }%
    \caption{(a) Our supernet architecture $\mathcal{S}$ and (b) a potential path $m$ selecting several module candidates $\mathcal{M}$.}%
\end{figure}

%
\begin{table}
    \begin{center}
    \caption{Deep neural network layer candidates.}
    \label{tab:candidates}   
    \scriptsize
    \begin{tabular}{|c|c|}
        \hline
        Index & Convolutional Operations \\
        \hline\hline
        1 & $3\times3\times3$ $3\mathcal{D}$ convolution\\
        \hline
        2 & $5\times5\times5$ $3\mathcal{D}$ convolution\\
        \hline
        3 & $7\times7\times7$ $3\mathcal{D}$ convolution\\
        \hline
        4 & $3\times3$ $2\mathcal{D}$ convolution on $\mathcal{X}$-direction\\
        \hline
        5 & $3\times3$ $2\mathcal{D}$ convolution on $\mathcal{Y}$-direction\\
        \hline
        6 & $3\times3$ $2\mathcal{D}$ convolution on $\mathcal{Z}$-direction\\
        \hline
        %7 & One $3\times3\times3$ $3\mathcal{D}$ residual block\\
        %\hline
        %8 & Two $3\times3\times3$ $3\mathcal{D}$ residual blocks\\
        %\hline
        %9 & Three $3\times3\times3$ $3\mathcal{D}$ residual blocks\\
        %\hline
    \end{tabular}
    \end{center}
\end{table}
%


==> old_miccai2020/03_Experiments.tex <==
\section{Experiments \& Results}
\label{sec:experiments}
Our proposed method is evaluated on the task of 3D whole prostate segmentation in T2-weighted MRI. In particular, MRI has challenges of data inconsistencies due to variations in the exact imaging protocols and scanners used at each data contributing site, potentially causing drastic variations in contrast and intensity values. 

\paragraph{\textbf{Datasets:}}
We utilize prostate MRI datasets from four different publicly available data sources. 
MSD-Prostate\footnote{\url{http://medicaldecathlon.com}} \cite{simpson2019large}, PROMISE12 \footnote{\url{https://promise12.grand-challenge.org}} \cite{litjens2014evaluation}, NCI-ISBI13\footnote{\url{http://doi.org/10.7937/K9/TCIA.2015.zF0vlOPv}}, and ProstateX\footnote{\url{https://prostatex.grand-challenge.org}} \cite{litjens2014computer}.
%
For each dataset, we perform three random splits into training, validation, and testing sets at roughly 70\%, 10\%, and 20\% of the total number of cases of each dataset. The resulting number of cases for each dataset are shown in Table \ref{tab:results}. We average results across the testing splits of each random split. For reference, we show the results on a centralized dataset where all four datasets have been combined. We also compare the performance for models trained locally and through federated learning an each dataset's testing split. The performance of standard 3D U-Net \cite{cciccek20163d} is shown for a baseline comparison. We resample each image to a constant resolution of 0.5 mm $\times$ 0.5 mm $\times$ 1.0 mm and normalize all non-zero image intensities by subtracting their mean and dividing by their standard derivation on a per-image basis. 

\paragraph{\textbf{Implementation:}}
Both U-Net and the supernet are trained using randomly cropped patches of size $256\times 256\times 32$ from the input images and labels. We used a mini-batch size of 4 by selecting two random crops from any two random input image and label pairs. As the optimizer for training the supernet, we chose \textit{NovoGrad} which has typically faster convergence speed than the more commonly used Adam optimizer \cite{ginsburg2019stochastic}. The learning rate for supernet training was set to $1e^{-2}$. For finding the optimal path for the final sub-network we use the Adam optimizer with a learning rate of $1e^{-3}$.
Augmentation techniques like random intensity shifts, contrast adjustments, and adding Gaussian noise are applied during training to avoid overfitting to the training set. Both 3D U-Net baseline and the supernet are implemented with PyTorch\footnote{\url{https://pytorch.org}} and trained on NVIDIA V100 GPUs with 32 GB memory.

\paragraph{\textbf{Results:}}
Table \ref{tab:results} and Fig. \ref{fig:results} show the performance for assuming both local, centrally hosted, and federated datasets. We show the performance of the proposed supernet training approach and its adaption to the local dataset distribution via path optimization, together with a baseline implementation of 3D U-Net using the same augmentation, optimization and hyperparameters to be comparable. All experiments used deterministic training with a fixed seed to guarantee comparable results. Sometimes, the locally optimal path $m_0 \in \mathcal{M}$ is equivalent to the based used for model selection during supernet training (the path with all $m=[1, 1, \dots, 1, 1]$ as shown in Table \ref{tab:candidates}). Hence, the numbers before and after adaption might be equivalent in Table \ref{tab:results} and Fig. \ref{fig:results}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%number train, valid, test, total:
%Centralised 172, 23, 48, 243
%Centralised 70.8, 9.5, 19.8 %
%NCI_ISBI 45, 6, 12, 63
%NCI_ISBI 71.4, 9.5, 19.0 %
%PROMISE12 35, 5, 10, 50
%PROMISE12 70.0, 10.0, 20.0 %
%PROSTATEx 69, 9, 20, 98
%PROSTATEx 70.4, 9.2, 20.4 %
%Task05_Prostate 23, 3, 6, 32
%Task05_Prostate 71.9, 9.4, 18.8 %
\begin{table*}[htbp]
    \caption{Results for centralized dataset and each dataset trained locally and in federated learning. We show the performance of a baseline 3D U-Net and our proposed supernet (SN) approach. The average Dice of the local model's scores is shown (excluding the scores on centralized data). The highest scores for each dataset are marked in \textbf{bold}.}
    \label{tab:results}
      \centering
      \footnotesize
      %\scriptsize
%\begin{tabular}{|l|l|l|l|l|l|l|}      
%\begin{tabular}{|p{25mm}|p{22mm}|p{22mm}|p{22mm}|p{22mm}|p{22mm}|p{22mm}|}
%\begin{tabular}{p{25mm}cccccc}
\begin{tabular}{lcccccc}
\hline\hline
\textbf{# Cases}& \textbf{Central} & \textbf{NCI}& \textbf{PROMISE12}& \textbf{ProstateX}& \textbf{MSD} & \\
\hline
# Training   & 172 & 45 & 35 & 69 & 23 \\
# Validation & 23  & 6  & 5  & 9  & 3  \\
# Testing    & 48  & 12 & 10 & 20 & 6  \\
\hline
# Total      & 243 & 63 & 50 & 98 & 32 \\
\hline\hline
      &  &  &  &  &  \\
\hline\hline
\textbf{Avg. Dice [\%]}& \textbf{Central} & \textbf{NCI}& \textbf{PROMISE12}& \textbf{ProstateX}& \textbf{MSD} & \textbf{Avg. (loc.)}\\
\hline
U-Net (loc.)        & \textbf{89.76} &	\textbf{89.62}	&	80.98	&	\textbf{91.75}	&	75.87	&	84.56 \\
U-Net (fed.)        &  	    &	83.71	&	81.74	&	90.61	&	77.05	&	83.28 \\
\hline
SN (loc.)           & 88.36 &	87.31	&	81.13	&	90.24	&	81.59	&	85.07 \\
SN (fed.)           &       &	88.79	&	85.35	&	91.45	&	\textbf{82.38}	&	86.99 \\
\hline
SN (loc.) + adapt.  & 89.02 &	88.75	&	81.72	&	90.33	&	80.77	&	85.39 \\
SN (fed.) + adapt.  & 	    &	88.60	&	\textbf{85.57}	&	91.45	&	\textbf{82.38}	&	\textbf{87.00} \\
\hline\hline
\end{tabular}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htbp]
 \centering
    \includegraphics[width=0.9\textwidth]{figs/Prostate_noAMP_eval_ep1_lr1e-3_bestonly_csvs.pdf} 
    \caption{The box plots show the distribution of Dice scores under each setting listed in Table \ref{tab:results} shown for one random test split for the different}%
    \label{fig:results}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> old_miccai2020/04_Conclusion.tex <==
\section{Discussion \& Conclusions}
\label{sec:conclusions}
It can be observed from Table \ref{tab:results} that the supernet training with local adaptation in FL \textit{(SN (fed.) + adapt.)} achieves the highest average Dice score on the local datasets. This illustrates the viability of supernet training with local model adaption to the client's data. We furthermore observe a general improvement of the local supernet models' performance when trained in an FL setting versus local training. This means that in particular supernet model training can benefit from the larger effective training set size made available through FL without having to share any of the raw image data between clients. The U-Net turned out to be a surprisingly strong baseline, sometimes outperforming the supernet approach in terms of average Dice numbers on a particular dataset. However, looking at the average local Dice scores, we can see a marked improvement when using the supernet. 
We can also observe an improvement in minimum Dice scores from \ref{fig:results} after local model adaption. This suggest that the locally adapted models are more robust to outlier cases that might be particular to a specific data source. Overall, the average Dice scores are comparable to recent literature on whole prostate segmentation in MRI \cite{litjens2014computer,litjens2014evaluation,milletari2016v} and can likely be improved with more aggressive data augmentation schemes \cite{zhang2020generalizing,isensee2018no,isensee2019nnu}.

In conclusion, we proposed to combine the advantages of both federated learning and AutoML approaches. The two techniques are complementary and in combination, they allow for an implicit domain adaptation through the finding of locally optimal model architectures (sub-networks of the supernet) for a client's dataset distribution. We showed that the performances of federated learning are comparable if not better than the model's performance when the dataset is centrally hosted. After local adaptation via choosing the optimal path through the supernet, we can see an additional performance gain on the client's data. In the future, it could be explored if there is a set of optimal sub-networks that could act as an ensemble during inference to further improve performance and provide additional estimates such as model uncertainty. Furthermore, one could adaptively change the path frequencies used during supernet training based on sub-network architectures that work well on each client.


%The results are comparable with recent work on whole prostate segmentation. For example, \cite{zhang2020generalizing} reports 91.9\% Dice achieved on the validation set of ProstateX with agressive data augmentation. In contraast while we achieve 91.45
